Steady-state nonlinearity of open-loop reset systems

In this paper, we introduce a new representation for open-loop reset systems. We show that at steady-state a reset integrator can be modelled as a parallel interconnection of the base-linear system and piece-wise constant nonlinearity. For sinusoidal input signals, this nonlinearity takes a form of a square wave. Subsequently, we show how the behaviour of a general open-loop reset system is related to the nonlinearity of a reset integrator. The proposed approach simplifies the analysis of reset elements in the frequency domain and provides new insights into the behaviour of reset control systems.

==> Sections/Derivations_backup.tex <==
\section{Nonlinearity of reset systems}
\label{sec:Derivations}

In order to analyse the steady-state behaviour of a system, we require it to be \textit{uniformly convergent} \cite{Pavlov2006a}\cite{Pavlov2007}. This condition is satisfied by reset system \eqref{eq:R}, for a class of sinusoidal inputs, if $|\lambda(A_\rho e^{A_r \delta})|<1, \foraal \delta\in\mathbb{R}^+$ \cite{Guo2009}.
%{\color{red}
%Note, that a double reset integrator does not satisfy this condition. It can be easily seen by considering the response of the BLS - it is not BIBO stable. However, we may be able to abuse the theory developed here and still calculate the steady-state response. 
%}
\begin{thm}[Reset integrator]\label{thm:Rint}
The steady-state state response of a well behaved reset integrator, i.e.\  reset system \eqref{eq:R} with $A_r = 0, B_r = I, C_r = I, D_r = 0$, to an input signal $u_r(t) = a \sin(\omega t)$ is given by 
\begin{equation}
    x_r(t) = x_{bls}(t) + q_i(t),
\end{equation}
where $x_{BLS}$ denotes the steady-state response of the base-linear system $(A_r,B_r,C_r,D_r)$ and $q_i$ is a square wave in phase with $u_r$, with peak amplitude
\begin{equation}
\hat q_i = \frac{I-A_\rho}{I + A_\rho}\frac{a}{\omega},
\end{equation}
and mean value (constant component)
\begin{equation}
\bar q_i = \frac{-a}{\omega}.
\end{equation}
\end{thm}

\begin{proof}
Consider dynamics of $q \triangleq x_r-x_{bls}$
\begin{equation}\label{eq:dq}
    \begin{cases}
    \dot q(t) = A_r q(t), & \text{if } u_r \neq 0\\
    q(t^+) = A_\rho q(t)+(A_\rho-I)x_{bls}(t), & \text{if } u_r = 0.
    \end{cases}
\end{equation}
It is clear that for a reset integrator $A_r  =0$ with any input $u_r$, $q(t)$ is piecewise constant, and jumps only at the reset instants.

$q(t)$ between consecutive reset instants $t_k,t_{k+1}$ is given by
\begin{equation}
    q(t) = q(t_k^+)+\int_{t_k}^t A_r q(\tau)\diff \tau, \text{ for } t\in(t_k, t_{k+1}).
\end{equation}
Note, that for a reset integrator we have $q_i(t) = q_i(t_k^+), t\in(t_k, t_{k+1})$ and $q_i(t_{k+1})  = q_i(t_k^+)$.

At a reset instant, for an input signal $u_r(t) = a \sin(\omega t)$, we have $t_{k} = k\frac{\pi}{\omega}, k\in \mathbb{N}$ and
\begin{equation}
\begin{split}
    q_i(t_k^+) &= 
    A_\rho q_i(t_{k-1}^+) + (A_\rho -I)\int_{t_{k-1}}^{t_{k}} B_r u_r(\tau) \diff \tau \\
    &= \begin{cases}
    A_\rho q_i(t_{2n}^+), & \text{if } k = 2n+1\\
    A_\rho q_i(t_{2n+1}^+) + (A_\rho -I)\frac{2a}{\omega}, & \text{if } k = 2n.
    \end{cases}
\end{split}    
\end{equation}
At the steady state, we have
\begin{equation}
    \begin{split}
        q_i(t_{2n}) &= q_i(t_{2n+2}^+)\\
        &= A_\rho q_i(t_{2n+1}^+)+(A_\rho -I)\frac{2a}{\omega} \\
        &= A_\rho^2 q_i(t_{2n}^+)+(A_\rho -I)\frac{2a}{\omega}
    \end{split}
\end{equation}
After solving for $q_i(t_{2n})$ we have
\begin{equation}
    q_i(t_{2n}^+) = \frac{A_\rho - I}{I-A_\rho^2}\frac{2a}{\omega} = \frac{-(I-A_\rho)}{(I-A_\rho)(I+A_\rho)}\frac{2a}{\omega} = \frac{-1}{I+A_\rho}\frac{2a}{\omega}.
\end{equation}
For $q_i(t_{2n+1}^+)$ we have
\begin{equation}
    q_i(t_{2n+1}^+) = \frac{-A_\rho}{I+A_\rho}\frac{2a}{\omega}.
\end{equation}

Taking all this into consideration we have 
\begin{equation}
    q_i(t) = 
    \begin{cases}
    \frac{-1}{I+A_\rho}\frac{2a}{\omega}, & \text{for } t \in [t_{2n},t_{2n+1})\\
    \frac{-A_\rho}{I+A_\rho}\frac{2a}{\omega}, & \text{for } t \in [t_{2n+1},t_{2n+2}).
    \end{cases}
\end{equation}

The mean value $\bar q$ and the peak amplitude $\hat q$ are given by
\begin{align}
    \bar q_i &= \frac{q(t_{2n}^+) + q(t_{2n+1}^+)}{2} = \frac{-a}{\omega}\\
    \hat q_i &= \frac{q(t_{2n+1}^+) - q(t_{2n}^+)}{2} = \frac{I-A_\rho}{I+A_\rho}\frac{a}{\omega}.
\end{align}

So we can also write
\begin{equation}
    q_i(t) = 
    \begin{cases}
    \bar q_i + \hat q_i, & \text{for } t \in [t_{2n},t_{2n+1})\\
    \bar q_i - \hat q_i, & \text{for } t \in [t_{2n+1},t_{2n+2}).
    \end{cases}
\end{equation}
\end{proof}

\begin{rem}
Signal $q(t)$ represents nonlinearity added to the system by the reset actions.
\end{rem}

\begin{thm}[Reset state-space system]
The steady-state state response of a well behaved reset system \eqref{eq:R} is given by 
\begin{align}
    x_{r} &= x_{bls} + q = x_{bls} + T_{q}*q_i,\\
    T_{q} &=\frac{x_r}{q_i}  = Q(sI-A_r)^{-1}s
\end{align}
where $x_{BLS}$ denotes the steady-state response of the base-linear system $(A_r,B_r,C_r,D_r)$ and $q_i$ is the square wave introduced in Theorem \ref{thm:Rint}, representing the nonlinearity in a reset integrator. 

The scaling of the magnitude of the the nonlinearity $Q\in \mathbb{R}^{m \times m}$ is given by
\begin{equation}
    \min_Q \left\lVert e^{A_r t}(I-A_\rho)x_{bls}(t_k)- e^{A_r t}A_\rho Q q^*(t_k)+Qq^*(t)\right\rVert_2^2,
\end{equation}
for $t\in (t_k,t_{k+1})$, where $t_k,t_{k+1}$ denote subsequent reset instants.
\end{thm}
\begin{proof}
Any state-space reset system can be represented in a block diagram form as a feedback system with a reset integrator and feedback gain $A_r$, see Fig. \ref{fig:Rss}. Using the Theorem \ref{thm:Rint}, the reset integrator can be represented as a parallel interconnection of its base-linear system and a block generating the signal related to reset. Reset instants of considered elements are depending only on the input signal. In consequence, reset instants for a reset integrator considered in Theorem \ref{thm:Rint} and a general reset state-space system are the same, if both  systems are driven by the same input signal.

\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/Rss.png}
  \caption{Block diagram representation of a reset state-space system. a) standard form, b) reset integrator represented in the BL+NL form, c) entire state-space element in the BL+NL form.}
  \label{fig:Rss}
\end{figure}

In Fig. \ref{fig:Rss} it can be seen that the state of a reset element consists of the response of the base linear system $x_{bls}$ and a contribution due to the nonlinearity $q_i$. This contribution is denoted by $q$ and defined in \eqref{eq:dq}. By analysing the block diagram b) in Fig. \ref{fig:Rss}, we have
\begin{align}
    x_r &= A_r\frac{I}{s}x_r + B_r\frac{I}{s} u_r + q,\\
    x_{r} &= x_{bls} + q = x_{bls} + T_{q}*q_i,\\
    T_{q} &=\frac{x_r}{q_i}  = Q(sI-A_r)^{-1}s
\end{align}

The transfer function (matrix) $T_{q}$ defines the shape of the nonlinear contribution. It can be represented in the state-space form by $(A_r,A_r,I,I)$. Placement of a reset integrator in a feedback system not only influences the shape of the nonlinear contribution, but also the amplitude, which is indicated by the term $Q\in \mathbb{R}^{m \times m}$.

To find the amplitude of the nonlinear contribution we consider evolution of a reset system states between reset instants. We define $q(t) \triangleq Q q^*(t), Q \in \mathbb{R}$. For $t\in (t_k,t_{k+1})$ we have
\begin{align}
x_r(t) = e^{A_r (t-t_k)}x_{bls}(t_k) + &{\int_{t_k}^t e^{A_r(t-\tau)}B_r u_r(\tau)\diff \tau} + q(t)\\
x_r(t) = e^{A_r (t-t_k)}x_{r}(t_k^+) &+ {\int_{t_k}^t e^{A_r(t-\tau)}B_r u_r(\tau)\diff \tau}\\
 e^{A_r(t-t_k)}x_{bls}(t_k) + q(t) = &e^{A_r(t-t_k)}x_{r}(t_k^+)\\
 e^{A_r(t-t_k)}x_{bls}(t_k) + Qq^*(t) = &e^{A_r(t-t_k)}A_\rho (x_{bls}(t_k)+Qq^*(t_k))\\
0 = e^{A_r t}(I-A_\rho)x_{bls}(t_k)- &e^{A_r t}A_\rho Q q^*(t_k)+Qq^*(t).
\end{align}
In consequence, $Q$ can be found as a solution for a minimization problem
\begin{equation}
    \min_Q \left\lVert e^{A_r t}(I-A_\rho)x_{bls}(t_k)- e^{A_r t}A_\rho Q q^*(t_k)+Qq^*(t)\right\rVert_2^2.
\end{equation}
If $m = 1$, it is sufficient to consider only the before and after-reset state. From \eqref{eq:dq} we have
\begin{align}
A_\rho x_r(t_k) &= x_{bls}(t_k) + q(t_k^+),\\
A_\rho \left(x_{bls}(t_k)+q(t_k)\right) &= x_{bls}(t_k) + q(t_k^+),\\
(A_\rho-I)x_{bls}(t_k) &= q(t_k^+) - A_\rho q(t_k),\\
(A_\rho-I)x_{bls}(t_k) &= Q\left(q^*(t_k^+) - A_\rho q^*(t_k)\right),\\
Q = (A_\rho-I) &x_{bls}(t_k)\big(q^*(t_k^+) - A_\rho q^*(t_k)\big) ^{-1}.
\end{align}
Consider response of $T_q$ to $q_i$
\begin{equation}\label{eq:q*t}
    q^*(t) = e^{A_r t}q^*(0) + \int_0^t e^{A_r(t-\tau)}A_r q_i(\tau)\diff \tau + q_i(t).
\end{equation}
At the steady state, the term related to $q^*(0)$ disappears. $q_i$ consists of a constant and a variable component. We have
\begin{equation}
    \int_0^t e^{A_r(t-\tau)}A_r \bar q_i\diff \tau = (e^{A_r t}-I)\bar q_i = -\bar q_i \text{ (for large $t$)}.
\end{equation}

Consider now $t \in [t_{2n}, t_{2n+1})$. The varying part $q_i(t) - \bar q_i$ is a zero-mean square wave with peak amplitude $\hat q_i$. We have
\begin{equation}
    \int_0^{t_{2n}} e^{A_r(t-\tau)}A_r (q_i(\tau) -\bar q_i)\diff \tau = 0
\end{equation}
The component due to the varying part for $t \in [t_{2n}, t_{2n+1})$ can be calculated as a response to step with magnitude $\hat q_i$. For this, we define the state of $T_q$ $x_q$, such that $q(t)^* = Ix_q(t) + Iq_i(t)$. The initial consition for the step is initial condition $x_q(t_{2n})$. At the steady state we have $x_q(t_{2n}) = -x_q(t_{2n+1})$ and
\begin{align}\label{eq:qtk}
    -e^{A_r \frac{\pi}{\omega}}x_q(t_{2n+1}) + (e^{A_r \frac{\pi}{\omega}}-I)\hat q = x_q(t_{2n+1})\\
    (e^{A_r \frac{\pi}{\omega}}+I)x_q(t_{2n+1}) = (e^{A_r \frac{\pi}{\omega}}-I)\hat q_i\\
    x_q(t_{2n+1}) = (e^{A_r \frac{\pi}{\omega}}+I)^{-1}(e^{A_r \frac{\pi}{\omega}}-I)\hat q_i\\
    q^*(t_{2n+1}) = \big((e^{A_r \frac{\pi}{\omega}}+I)^{-1}(e^{A_r \frac{\pi}{\omega}}-I) +I \big)\hat q_i
\end{align}
The value of $q^*(t)$ during the after-reset flow $t\in (t_{2n+1}, t_{2n+2})$ can be found as a response to step with magnitude $-\hat q_i$. The after reset value $q^*(t_{2n+1}^+)$ is given by
\begin{align}\label{eq:qtk+}
    %x_q(t_{2n+1}^+) = e^{A_r 0}(x_q(t_{2n+1})+A_r \hat q_i) = x_q(t_{2n+1})+A_r \hat q_i\\
    q^*(t_{2n+1}^+) = x_q(t_{2n+1})-I\hat q_i.
\end{align}

The response of the base-linear system at a reset instant is given by
\begin{equation}
\begin{split}
    x_{bls}(t_k) &= e^{A_r t}x_{bls}(0) + \int_0^t e^{A_r(t-\tau)}B_r a \sin(\omega \tau)\diff \tau \\ &= \begin{cases} 
    ~~(A_r^2+\omega^2I)^{-1}B_r a\omega, \text{ for } k = 2n+1\\
    -(A_r^2+\omega^2I)^{-1}B_r a\omega, \text{ for } k = 2n+2.
    \end{cases}
\end{split}
\end{equation}
\end{proof}

The following corollaries are a consequence of the fact that an ideal square wave can be represented as an infinite sum of sinusoidal waves
\begin{equation}
    q_i(t) = \bar q_i + \hat q_i \frac{4}{\pi}\left(\sin(\omega t) + \frac{1}{3}\sin(3\omega t)+\frac{1}{5}\sin(5\omega t)\dots \right).
\end{equation}

\begin{cor}\label{cor:qharmonics}
The $k$-th harmonic of the nonlinear contribution $q$ in the reset system \eqref{eq:R} is given  by 
\begin{equation}
    q_k(\omega) = 
    \begin{cases}
     \frac{4}{k\pi}C_rQ(jk\omega I - A_r)^{-1}jk\omega \hat g_i J_{n,1} & \text{for odd } k\\
     0 &\text{for even } k
    \end{cases}
\end{equation}
where $J_{m,1}$ denotes a vector of ones with an appropriate size.
\end{cor}

\begin{cor}\label{cor:HOSIDF}
The Higher-order Sinusoidal-input Describing function (HOSIDF) of the reset system \eqref{eq:R} is given  by 
\begin{equation}
    H_k(\omega) = 
    \begin{cases}
    C_r\left(j\omega I-A_r\right)^{-1}B_r+D_r + q_1(\omega) & \text{for } k=1\\
     q_k(\omega) & \text{for } k\geq 2
    \end{cases}
\end{equation}
\end{cor}
Corollaries \ref{cor:qharmonics} and \ref{cor:HOSIDF} give a clear insight into the behaviour of HOSIDF for reset elements.

